3D Scene Understanding Through Local Random Access Sequence Modeling

3D scene understanding from single images is a pivotal problem in computer vision with numerous downstream applications in graphics, augmented reality, and robotics. While diffusion-based modeling approaches have shown promise, they often struggle to maintain object and scene consistency, especially in complex real-world scenarios. To address these limitations, we propose an autoregressive generative approach called Local Random Access Sequence (LRAS) modeling, which uses local patch quantization and randomly ordered sequence generation. By utilizing optical flow as an intermediate representation for 3D scene editing, our experiments demonstrate that LRAS achieves state-of-the-art novel view synthesis and 3D object manipulation capabilities. Furthermore, we show that our framework naturally extends to self-supervised depth estimation through a simple modification of the sequence design. By achieving strong performance on multiple 3D scene understanding tasks, LRAS provides a unified and effective framework for building the next generation of 3D vision models.

==> tables/depth_dynamic.tex <==

% AbsRel Log10 RMS
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.2} % Adjust row height for readability
    \setlength{\tabcolsep}{6pt} % Adjust column spacing
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Model} & \textbf{AbsRel} $\downarrow$ & \textbf{Log10} $\downarrow$ & \textbf{RMSE} $\downarrow$ & \textbf{$\delta_1$} $\uparrow$ & \textbf{$\delta_2$} $\uparrow$ & \textbf{$\delta_3$} $\uparrow$ \\
        \midrule
        SC-Depth-V2  & 1.000  & 1.000  & 1.000  & 1.000  & 1.000 & 1.000  \\
        % MotionCtrl   & 1.000  & 1.000  & 1.000  & 1.000  & 1.000  \\
        IndoorDepth  & 1.000  & 1.000  & 1.000  & 1.000  & 1.000 & 1.000  \\
        \midrule
        \textbf{PSI (Ours)} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
        \bottomrule
    \end{tabular}
    \captionsetup{labelfont=bf}
    \caption{Comparison of self-supervised depth estimation models on NYUD. Lower is better for AbsRel and RMSE ($\downarrow$), while higher is better for $\delta_1$, $\delta_2$, and $\delta_3$ ($\uparrow$).}
    \label{tab:depth_comparison}
\end{table}



==> tables/nvs_decoding_order.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.2} % Adjust row height for readability
    \setlength{\tabcolsep}{6pt} % Adjust column spacing
    \begin{tabular}{lccc}
        \toprule
        \textbf{Dataset} \\
        \textbf{Model} & \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ & \textbf{LPIPS} $\downarrow$ \\
        \midrule
        \textbf{WildRGB-D} \\
        LRAS w. Scanning Order  & 17.702 & 0.537 & 0.221 \\
        LRAS w. Random Order & 17.895  & 0.541 & 0.231 \\
        % \midrule
        % \textbf{DL3DV} \\
        % Ours w. Our Depth  & 18.169  & 0.524  & 0.324 \\
        % Ours w. DepthAnythingv2 & 18.279 & 0.531 & 0.321 \\
        \bottomrule
        
    \end{tabular}
    \caption{Comparison of Different Decoding Orders.}
    \label{tab:nvs_decoding_order}
\end{table}

==> tables/nvs_our_depth_v0.tex <==

% \begin{table}[h]
%     \centering
%     \renewcommand{\arraystretch}{1.2} % Adjust row height for readability
%     \setlength{\tabcolsep}{4pt} % Adjust column spacing
%     \begin{tabular}{lccc}
%         \toprule
%         \textbf{Dataset} \\
%         \textbf{Model} & \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ & \textbf{LPIPS} $\downarrow$ \\
%         \midrule
%         \textbf{WildRGB-D} \\
%         LRAS \newline w. Our Depth  & 16.903 & 0.491 & 0.257 \\
%         LRAS \newline w. DepthAnythingv2 & 17.895  & 0.541 & 0.231 \\
%         \midrule
%         \textbf{DL3DV} \\
%         Ours w. Our Depth  & 18.169  & 0.524  & 0.324 \\
%         Ours w. DepthAnythingv2 & 18.279 & 0.531 & 0.321 \\
%         \bottomrule
        
%     \end{tabular}
%     \captionsetup{labelfont=bf}
%     \caption{\textbf{Comparison of metrics for novel view synthesis depending on depth model.}}
%     \label{tab:nvs_our_depth}
% \end{table}

\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.2} % Adjust row height for readability
    \setlength{\tabcolsep}{4pt} % Adjust column spacing
    \begin{tabular}{llccc}
        \toprule
        \textbf{Dataset} & \textbf{LRAS} & \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ & \textbf{LPIPS} $\downarrow$ \\
        \midrule
        \multirow{2}{*}{\textbf{WildRGB-D}} 
        & \makecell[l]{w. Our Depth}  & 16.903 & 0.491 & 0.257 \\
        & \makecell[l]{w. DAv2} & \textbf{17.895}  & \textbf{0.541} & \textbf{0.231} \\
        \midrule
        \multirow{2}{*}{\textbf{DL3DV}} 
        & \makecell[l]{w. Our Depth}  & 18.169  & 0.524  & 0.324 \\
        & \makecell[l]{w. DAv2} & \textbf{18.279} & \textbf{0.531} & \textbf{0.321} \\
        \bottomrule
    \end{tabular}
    \captionsetup{labelfont=bf}
    \caption{\textbf{Comparison of metrics for novel view synthesis depending on depth model.}}
    \label{tab:nvs_our_depth}
\end{table}


% \begin{table}[h]
%     \centering
%     \renewcommand{\arraystretch}{1.2} % Adjust row height for readability
%     \setlength{\tabcolsep}{6pt} % Adjust column spacing
%     \begin{tabular}{lcccc}
%         \toprule
%         \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{WildRGB-D}} & \multicolumn{2}{c}{\textbf{DL3DV}} \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%          & \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ & \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ \\
%         \midrule
%         ZeroNVS      & 21.12  & 0.874  & 22.35  & 0.891 \\
%         ViewCrafter  & 22.98  & 0.895  & 23.47  & 0.902 \\
%         \midrule
%         \textbf{PSI (Ours)} & \textbf{24.12} & \textbf{0.910} & \textbf{25.01} & \textbf{0.920} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Comparison of Novel View Synthesis models on WildRGB-D and DL3DV datasets. Higher is better for PSNR and SSIM ($\uparrow$).}
%     \label{tab:nvs}
% \end{table}

==> tables/nvs_v0.tex <==

% \begin{table}[t]
%     \centering
%     \renewcommand{\arraystretch}{1.2} % Adjust row height for readability
%     \setlength{\tabcolsep}{6pt} % Adjust column spacing
%     \begin{tabular}{lccc}
%         \toprule
%         \textbf{Dataset} \\
%         \textbf{Model} & \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ & \textbf{LPIPS} $\downarrow$ \\
%         \midrule
%         \textbf{WildRGB-D} \\
%         MotionCtrl & 13.117 & 0.321 & 0.355 \\
%         ZeroNVS  & 16.418  & 0.470  & 0.276 \\
%         ViewCrafter  & 14.138  & 0.383  & 0.280 \\
%         \textbf{LRAS(Ours)} & \textbf{17.895}  & \textbf{0.541} & \textbf{0.231} \\
%         \midrule
%         \textbf{DL3DV} \\
%         MotionCtrl & 12.629 & 0.261 & 0.462 \\
%         ZeroNVS  & 15.950  & 0.417  & 0.323 \\
%         ViewCrafter  & 16.738  & 0.437  & \textbf{0.247} \\
%         \textbf{LRAS(Ours)} & \textbf{18.279} & \textbf{0.531} & 0.321 \\
%         \bottomrule
        
%     \end{tabular}
%     \captionsetup{labelfont=bf}
%     \caption{\textbf{Comparison of metrics for novel view synthesis.}}
%     \label{tab:nvs}
% \end{table}


\begin{table}[t]
    \centering
    \renewcommand{\arraystretch}{1.2} % Adjust row height for readability
    \setlength{\tabcolsep}{4pt} % Adjust column spacing
    % \captionsetup{labelfont=bf}
    \begin{tabular}{llccc}
        \toprule
        \textbf{Dataset} & \textbf{Model} & \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ & \textbf{LPIPS} $\downarrow$ \\
        \midrule
        \multirow{4}{*}{\textbf{WildRGB-D}} 
        & MotionCtrl & 12.394 & 0.293 & 0.404 \\
        & ZeroNVS  & 16.418  & 0.470  & 0.276 \\
        & ViewCrafter  & 14.138  & 0.383  & 0.280 \\
        & \textbf{LRAS (Ours)} & \textbf{17.895}  & \textbf{0.541} & \textbf{0.231} \\
        \midrule
        \multirow{4}{*}{\textbf{DL3DV}} 
        & MotionCtrl & 12.629 & 0.261 & 0.462 \\
        & ZeroNVS  & 15.950  & 0.417  & 0.323 \\
        & ViewCrafter  & 16.738  & 0.437  & \textbf{0.247} \\
        & \textbf{LRAS (Ours)} & \textbf{18.279} & \textbf{0.531} & 0.321 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison of metrics for novel view synthesis.}}
    \label{tab:nvs}
\end{table}



 % on WildRGB-D and DL3DV datasets.

% \begin{table}[h]
%     \centering
%     \renewcommand{\arraystretch}{1.2} % Adjust row height for readability
%     \setlength{\tabcolsep}{6pt} % Adjust column spacing
%     \begin{tabular}{lcccc}
%         \toprule
%         \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{WildRGB-D}} & \multicolumn{2}{c}{\textbf{DL3DV}} \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%          & \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ & \textbf{PSNR} $\uparrow$ & \textbf{SSIM} $\uparrow$ \\
%         \midrule
%         ZeroNVS      & 21.12  & 0.874  & 22.35  & 0.891 \\
%         ViewCrafter  & 22.98  & 0.895  & 23.47  & 0.902 \\
%         \midrule
%         \textbf{PSI (Ours)} & \textbf{24.12} & \textbf{0.910} & \textbf{25.01} & \textbf{0.920} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Comparison of Novel View Synthesis models on WildRGB-D and DL3DV datasets. Higher is better for PSNR and SSIM ($\uparrow$).}
%     \label{tab:nvs}
% \end{table}
